From Dense to Sparse: Event Response for Enhanced Residential Load Forecasting

Residential load forecasting (RLF) is crucial for resource scheduling in power systems. Most existing methods utilize all given load records (dense data) to indiscriminately extract the dependencies between historical and future time series. However, there exist important regular patterns residing in the event-related associations among different appliances (sparse knowledge), which have yet been ignored. In this paper, we propose an Event-Response Knowledge Guided approach (ERKG) for RLF by incorporating the estimation of electricity usage events for different appliances, mining event-related sparse knowledge from the load series. With ERKG, the event-response estimation enables portraying the electricity consumption behaviors of residents, revealing regular variations in appliance operational states. To be specific, ERKG consists of knowledge extraction and guidance: i) a forecasting model is designed for the electricity usage events by estimating appliance operational states, aiming to extract the event-related sparse knowledge; ii) a novel knowledge-guided mechanism is established by fusing such state estimates of the appliance events into the RLF model, which can give particular focuses on the patterns of users' electricity consumption behaviors. Notably, ERKG can flexibly serve as a plug-in module to boost the capability of existing forecasting models by leveraging event response. In numerical experiments, extensive comparisons and ablation studies have verified the effectiveness of our ERKG, e.g., over 8% MAE can be reduced on the tested state-of-the-art forecasting models.

==> src/table/ablation_table.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Add caption}
    \begin{tabular}{cc||rr|rr|rr|rr}
    \toprule
    \multicolumn{2}{c}{Dataset} & \multicolumn{2}{c}{Ampds2} & \multicolumn{2}{c}{UK-DALEh1} & \multicolumn{2}{c}{UMASS3} & \multicolumn{2}{c}{UMASS4} \\
    \midrule
    \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
    \midrule
    \midrule
    \multirow{5}[2]{*}{origin} & 6     &       &       &       &       &       &       &       &  \\
          & 12    &       &       &       &       &       &       &       &  \\
          & 24    &       &       &       &       &       &       &       &  \\
          & 60    &       &       &       &       &       &       &       &  \\
          & 168   &       &       &       &       &       &       &       &  \\
    \midrule
    \multirow{5}[2]{*}{SP+H} & 6     &       &       &       &       &       &       &       &  \\
          & 12    &       &       &       &       &       &       &       &  \\
          & 24    &       &       &       &       &       &       &       &  \\
          & 60    &       &       &       &       &       &       &       &  \\
          & 168   &       &       &       &       &       &       &       &  \\
    \midrule
    \multirow{5}[2]{*}{mps+HF} & 6     &       &       &       &       &       &       &       &  \\
          & 12    &       &       &       &       &       &       &       &  \\
          & 24    &       &       &       &       &       &       &       &  \\
          & 60    &       &       &       &       &       &       &       &  \\
          & 168   &       &       &       &       &       &       &       &  \\
    \midrule
    \multirow{5}[2]{*}{SP+PF} & 6     &       &       &       &       &       &       &       &  \\
          & 12    &       &       &       &       &       &       &       &  \\
          & 24    &       &       &       &       &       &       &       &  \\
          & 60    &       &       &       &       &       &       &       &  \\
          & 168   &       &       &       &       &       &       &       &  \\
    \midrule
    \multirow{5}[2]{*}{MPS+PF(ours)} & 6     &       &       &       &       &       &       &       &  \\
          & 12    &       &       &       &       &       &       &       &  \\
          & 24    &       &       &       &       &       &       &       &  \\
          & 60    &       &       &       &       &       &       &       &  \\
          & 168   &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> src/table/ablation_wo_response.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Ablation without response based knowledge fusing}
    \begin{tabular}{c|c||cccccc}
    \toprule
    \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{origin} & \multicolumn{2}{c}{without response} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
    \midrule
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}} & 1     & 0.440  & 0.884  & 0.490  & 1.029  & \textbf{0.397 } & \textbf{0.775 } \\
          & 6     & 0.479  & 0.992  & 0.495  & 1.013  & \textbf{0.435 } & \textbf{0.850 } \\
          & 12    & 0.494  & 1.015  & 0.506  & 1.025  & \textbf{0.445 } & \textbf{0.869 } \\
          & 24    & 0.490  & 1.019  & 0.502  & 1.039  & \textbf{0.448 } & \textbf{0.874 } \\
          & 36    & 0.496  & 1.009  & 0.518  & 1.036  & \textbf{0.448 } & \textbf{0.882 } \\
          & 48    & 0.497  & 1.021  & 0.514  & 1.066  & \textbf{0.450 } & \textbf{0.881 } \\
          & 60    & 0.495  & 1.018  & 0.521  & 1.063  & \textbf{0.445 } & \textbf{0.863 } \\
          & 72    & 0.500  & 1.021  & 0.515  & 1.049  & \textbf{0.457 } & \textbf{0.907 } \\
          & 168   & 0.506  & 1.024  & 0.536  & 1.088  & \textbf{0.470 } & \textbf{0.901 } \\
          & 336   & 0.514  & 1.049  & 0.547  & 1.075  & \textbf{0.472 } & \textbf{0.896 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}} & 1     & 0.488  & 0.958  & 0.490  & 0.982  & \textbf{0.460 } & \textbf{0.918 } \\
          & 6     & 0.561  & 1.062  & 0.564  & 1.068  & \textbf{0.536 } & \textbf{1.039 } \\
          & 12    & 0.587  & 1.080  & 0.601  & 1.104  & \textbf{0.565 } & \textbf{1.049 } \\
          & 24    & 0.600  & 1.104  & 0.599  & 1.108  & \textbf{0.562 } & \textbf{1.081 } \\
          & 36    & 0.610  & 1.138  & 0.606  & 1.129  & \textbf{0.556 } & \textbf{1.071 } \\
          & 48    & 0.595  & 1.114  & 0.591  & 1.135  & \textbf{0.547 } & \textbf{1.071 } \\
          & 60    & 0.591  & 1.139  & 0.601  & 1.133  & \textbf{0.548 } & \textbf{1.076 } \\
          & 72    & 0.589  & 1.129  & 0.593  & 1.135  & \textbf{0.540 } & \textbf{1.068 } \\
          & 168   & 0.574  & 1.147  & 0.592  & 1.136  & \textbf{0.518 } & \textbf{1.060 } \\
          & 336   & 0.567  & 1.141  & 0.568  & 1.131  & \textbf{0.515 } & \textbf{1.062 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Umass3\end{sideways}} & 1     & 0.490  & 1.032  & 0.508  & 1.071  & \textbf{0.439 } & \textbf{0.928 } \\
          & 6     & 0.577  & 1.167  & 0.587  & 1.188  & \textbf{0.518 } & \textbf{1.067 } \\
          & 12    & 0.603  & 1.213  & 0.609  & 1.188  & \textbf{0.514 } & \textbf{1.061 } \\
          & 24    & 0.596  & 1.193  & 0.591  & 1.206  & \textbf{0.530 } & \textbf{1.079 } \\
          & 36    & 0.603  & 1.200  & 0.609  & 1.207  & \textbf{0.524 } & \textbf{1.064 } \\
          & 48    & 0.607  & 1.208  & 0.615  & 1.189  & \textbf{0.507 } & \textbf{1.060 } \\
          & 60    & 0.605  & 1.223  & 0.607  & 1.235  & \textbf{0.533 } & \textbf{1.111 } \\
          & 72    & 0.624  & 1.243  & 0.628  & 1.252  & \textbf{0.516 } & \textbf{1.089 } \\
          & 168   & 0.613  & 1.226  & 0.627  & 1.221  & \textbf{0.516 } & \textbf{1.066 } \\
          & 336   & 0.624  & 1.221  & 0.625  & 1.253  & \textbf{0.555 } & \textbf{1.080 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Umass4\end{sideways}} & 1     & 0.354  & 0.719  & 0.376  & 0.739  & \textbf{0.322 } & \textbf{0.674 } \\
          & 6     & 0.430  & 0.846  & 0.445  & 0.839  & \textbf{0.386 } & \textbf{0.773 } \\
          & 12    & 0.466  & 0.869  & 0.450  & 0.851  & \textbf{0.430 } & \textbf{0.806 } \\
          & 24    & 0.451  & 0.860  & 0.461  & 0.860  & \textbf{0.429 } & \textbf{0.817 } \\
          & 36    & 0.519  & 0.892  & 0.490  & 0.880  & \textbf{0.442 } & \textbf{0.830 } \\
          & 48    & 0.477  & 0.888  & 0.478  & 0.902  & \textbf{0.439 } & \textbf{0.837 } \\
          & 60    & 0.522  & 0.899  & 0.517  & 0.908  & \textbf{0.492 } & \textbf{0.843 } \\
          & 72    & 0.485  & 0.886  & 0.508  & 0.893  & \textbf{0.484 } & \textbf{0.830 } \\
          & 168   & 0.527  & 0.915  & \textbf{0.482 } & 0.905  & 0.484  & \textbf{0.850 } \\
          & 336   & \textbf{0.475 } & 0.887  & 0.482  & 0.887  & 0.493  & \textbf{0.858 } \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%

==> src/table/ablation_wo_share.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Ablation without MSP}
    \begin{tabular}{c|c||ccrrcc}
    \toprule
    \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{origin} & \multicolumn{2}{c}{without MSP} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
    \midrule
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}} & 1     & 0.440  & 0.884  & 0.406  & 0.800  & \textbf{0.397 } & \textbf{0.775 } \\
          & 6     & 0.479  & 0.992  & 0.435  & 0.842  & \textbf{0.435 } & \textbf{0.850 } \\
          & 12    & 0.494  & 1.015  & 0.460  & 0.924  & \textbf{0.445 } & \textbf{0.869 } \\
          & 24    & 0.490  & 1.019  & 0.450  & 0.892  & \textbf{0.448 } & \textbf{0.874 } \\
          & 36    & 0.496  & 1.009  & 0.456  & 0.903  & \textbf{0.448 } & \textbf{0.882 } \\
          & 48    & 0.497  & 1.021  & 0.452  & 0.885  & \textbf{0.450 } & \textbf{0.881 } \\
          & 60    & 0.495  & 1.018  & 0.457  & 0.893  & \textbf{0.445 } & \textbf{0.863 } \\
          & 72    & 0.500  & 1.021  & \textbf{0.453 } & \textbf{0.903 } & 0.457  & 0.907  \\
          & 168   & 0.506  & 1.024  & \textbf{0.463 } & \textbf{0.889 } & 0.470  & 0.901  \\
          & 336   & 0.514  & 1.049  & 0.485  & 0.930  & \textbf{0.472 } & \textbf{0.896 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}} & 1     & 0.488  & 0.958  & 0.465  & 0.933  & \textbf{0.460 } & \textbf{0.918 } \\
          & 6     & 0.561  & 1.062  & \textbf{0.534 } & \textbf{1.036 } & 0.536  & 1.039  \\
          & 12    & 0.587  & 1.080  & \textbf{0.554 } & 1.055  & 0.565  & \textbf{1.049 } \\
          & 24    & 0.600  & 1.104  & 0.571  & \textbf{1.063 } & \textbf{0.562 } & 1.081  \\
          & 36    & 0.610  & 1.138  & 0.577  & 1.081  & \textbf{0.556 } & \textbf{1.071 } \\
          & 48    & 0.595  & 1.114  & 0.547  & 1.072  & \textbf{0.547 } & \textbf{1.071 } \\
          & 60    & 0.591  & 1.139  & 0.560  & \textbf{1.072 } & \textbf{0.548 } & 1.076  \\
          & 72    & 0.589  & 1.129  & 0.548  & 1.076  & \textbf{0.540 } & \textbf{1.068 } \\
          & 168   & 0.574  & 1.147  & 0.527  & \textbf{1.058 } & \textbf{0.518 } & 1.060  \\
          & 336   & 0.567  & 1.141  & 0.525  & 1.067  & \textbf{0.515 } & \textbf{1.062 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Umass3\end{sideways}} & 1     & 0.490  & 1.032  & 0.461  & 0.966  & \textbf{0.439 } & \textbf{0.928 } \\
          & 6     & 0.577  & 1.167  & 0.538  & 1.079  & \textbf{0.518 } & \textbf{1.067 } \\
          & 12    & 0.603  & 1.213  & 0.549  & 1.111  & \textbf{0.514 } & \textbf{1.061 } \\
          & 24    & 0.596  & 1.193  & 0.513  & 1.095  & \textbf{0.530 } & \textbf{1.079 } \\
          & 36    & 0.603  & 1.200  & \textbf{0.534 } & 1.094  & 0.524  & \textbf{1.064 } \\
          & 48    & 0.607  & 1.208  & 0.562  & 1.107  & \textbf{0.507 } & \textbf{1.060 } \\
          & 60    & 0.605  & 1.223  & 0.583  & 1.124  & \textbf{0.533 } & \textbf{1.111 } \\
          & 72    & 0.624  & 1.243  & 0.556  & 1.120  & \textbf{0.516 } & \textbf{1.089 } \\
          & 168   & 0.613  & 1.226  & 0.538  & 1.097  & \textbf{0.516 } & \textbf{1.066 } \\
          & 336   & 0.624  & 1.221  & \textbf{0.543 } & 1.093  & 0.555  & \textbf{1.080 } \\
    \midrule
    \multirow{10}[2]{*}{\begin{sideways}Umass4\end{sideways}} & 1     & 0.354  & 0.719  & 0.326  & 0.688  & \textbf{0.322 } & \textbf{0.674 } \\
          & 6     & 0.430  & 0.846  & 0.397  & 0.778  & \textbf{0.386 } & \textbf{0.773 } \\
          & 12    & 0.466  & 0.869  & \textbf{0.425 } & \textbf{0.799 } & 0.430  & \textbf{0.806 } \\
          & 24    & 0.451  & 0.860  & 0.460  & 0.817  & \textbf{0.429 } & \textbf{0.817 } \\
          & 36    & 0.519  & 0.892  & 0.469  & \textbf{0.821 } & \textbf{0.442 } & \textbf{0.830 } \\
          & 48    & 0.477  & 0.888  & 0.439  & \textbf{0.817 } & \textbf{0.439 } & \textbf{0.837 } \\
          & 60    & 0.522  & 0.899  & \textbf{0.464 } & \textbf{0.826 } & 0.492  & \textbf{0.843 } \\
          & 72    & 0.485  & 0.886  & 0.489  & 0.852  & \textbf{0.484 } & \textbf{0.830 } \\
          & 168   & 0.527  & 0.915  & \textbf{0.477 } & 0.865  & 0.484  & \textbf{0.850 } \\
          & 336   & \textbf{0.475 } & 0.887  & 0.494  & \textbf{0.849 } & 0.493  & 0.858  \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table}%


==> src/table/average_horizon_without_msp.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Ablation without MSP: the average metric which prediction length in[1,6,12,24,36,48,60,72,168,336]}
    \begin{tabular}{c||cccccc}
    \toprule
    \multicolumn{1}{c}{Method} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{w/o MSP} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{1}{c}{Metric} & MAE   & MAPE` & MAE   & MAPE` & MAE   & MAPE` \\
    \midrule
    \midrule
    Ampds2 & 0.491  & 1.005  & 0.452  & 0.886  & \textbf{0.447 } & \textbf{0.870 } \\
    UK-DALEh1 & 0.576  & 1.101  & 0.541  & 1.051  & \textbf{0.535 } & \textbf{1.049 } \\
    Umass3 & 0.594  & 1.193  & 0.538  & 1.089  & \textbf{0.515 } & \textbf{1.060 } \\
    Umass4 & 0.471  & 0.866  & 0.444  & \textbf{0.811 } & \textbf{0.440 } & 0.812  \\
    \bottomrule
    \end{tabular}%
  \label{tab:blation without MSP}%
\end{table}%

==> src/table/average_horizon_without_response.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Ablation without response loss: the average metric which horizon in[1,6,12,24,36,48,60,72,168,336}
    \begin{tabular}{c||cccccc}
    \toprule
    \multicolumn{1}{c}{Method} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{w/o response loss} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{1}{c}{Metric} & MAE   & MAPE` & MAE   & MAPE` & MAE   & MAPE` \\
    \midrule
    \midrule
    Ampds2 & 0.491  & 1.005  & 0.515  & 1.048  & \textbf{0.447 } & \textbf{0.870 } \\
    UK-DALEh1 & 0.576  & 1.101  & 0.580  & 1.106  & \textbf{0.535 } & \textbf{1.049 } \\
    Umass3 & 0.594  & 1.193  & 0.601  & 1.201  & \textbf{0.515 } & \textbf{1.060 } \\
    Umass4 & 0.471  & 0.866  & 0.469  & 0.866  & \textbf{0.440 } & \textbf{0.812 } \\
    \bottomrule
    \end{tabular}%
  \label{tab:Ablation without response}%
\end{table}%


==> src/table/indicators_combine2.tex <==
% Table generated by Excel2LaTeX from sheet 'indicators_combine2'
  \centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{rrrrrrrrrrrrrrrrrrrrrrrrrrrrr} 
          & \multicolumn{1}{l}{mae} & \multicolumn{1}{l}{mae} & \multicolumn{1}{l}{mae} & \multicolumn{1}{l}{mae} & \multicolumn{1}{l}{mse} & \multicolumn{1}{l}{mse} & \multicolumn{1}{l}{mse} & \multicolumn{1}{l}{mse} & \multicolumn{1}{l}{rmse} & \multicolumn{1}{l}{rmse} & \multicolumn{1}{l}{rmse} & \multicolumn{1}{l}{rmse} & \multicolumn{1}{l}{smape} & \multicolumn{1}{l}{smape} & \multicolumn{1}{l}{smape} & \multicolumn{1}{l}{smape} & \multicolumn{1}{l}{mspe} & \multicolumn{1}{l}{mspe} & \multicolumn{1}{l}{mspe} & \multicolumn{1}{l}{mspe} & \multicolumn{1}{l}{rse} & \multicolumn{1}{l}{rse} & \multicolumn{1}{l}{rse} & \multicolumn{1}{l}{rse} & \multicolumn{1}{l}{corr} & \multicolumn{1}{l}{corr} & \multicolumn{1}{l}{corr} & \multicolumn{1}{l}{corr} \\ 
          & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} & \multicolumn{1}{l}{crossformer} & \multicolumn{1}{l}{crossformer\_origin} & \multicolumn{1}{l}{etsformer} & \multicolumn{1}{l}{etsformer\_origin} \\ 
    1     & 0.353186 & 0.379045 & 0.40994 & 0.443208 & 0.649614 & 0.629421 & 0.723919 & 0.702421 & 0.794208 & 0.782219 & 0.840469 & 0.828433 & 0.657576 & 0.744118 & 0.824219 & 0.913181 & 594.5658 & 397.1786 & 881.7889 & 567.9569 & 0.583094 & 0.574835 & 0.618816 & 0.610197 & 0.53227 & 0.546191 & 0.460919 & 0.465941 \\ 
    6     & 0.39786 & 0.419628 & 0.445907 & 0.491772 & 0.787731 & 0.774626 & 0.867382 & 0.853564 & 0.875979 & 0.868924 & 0.921071 & 0.913471 & 0.794993 & 0.841213 & 0.88128 & 1.007799 & 245.0325 & 983.4619 & 976.8374 & 1622.813 & 0.644671 & 0.63948 & 0.678836 & 0.673043 & 0.3834 & 0.388043 & 0.30995 & 0.305508 \\ 
    12    & 0.412676 & 0.434503 & 0.453397 & 0.504202 & 0.818531 & 0.800447 & 0.884738 & 0.873919 & 0.893549 & 0.883898 & 0.930169 & 0.924663 & 0.807471 & 0.887246 & 0.897601 & 1.038892 & 620.7146 & 327.2342 & 883.8563 & 1420.536 & 0.657659 & 0.650636 & 0.685001 & 0.681364 & 0.359884 & 0.363431 & 0.291748 & 0.285426 \\ 
    24    & 0.410157 & 0.429316 & 0.452095 & 0.507062 & 0.831367 & 0.819405 & 0.890063 & 0.890231 & 0.900136 & 0.894026 & 0.932438 & 0.933145 & 0.791956 & 0.80572 & 0.897947 & 1.04376 & 775.633 & 375.0617 & 1230.976 & 1512.688 & 0.661815 & 0.657545 & 0.685907 & 0.687296 & 0.34701 & 0.345887 & 0.284001 & 0.285002 \\ 
    36    & 0.409904 & 0.4493 & 0.451146 & 0.510339 & 0.841617 & 0.823835 & 0.893938 & 0.911457 & 0.905239 & 0.895906 & 0.933987 & 0.943437 & 0.748952 & 0.938692 & 0.88549 & 1.031941 & 332.6111 & 389.3035 & 400.7425 & 1322.781 & 0.66487 & 0.658082 & 0.686638 & 0.694041 & 0.339223 & 0.344196 & 0.289643 & 0.282397 \\ 
    48    & 0.419662 & 0.446434 & 0.45259 & 0.504888 & 0.845947 & 0.826786 & 0.90995 & 0.904684 & 0.908405 & 0.898469 & 0.94301 & 0.940275 & 0.837961 & 0.925181 & 0.890444 & 1.032709 & 258.7647 & 487.2564 & 521.9476 & 1306.03 & 0.666871 & 0.659682 & 0.692873 & 0.691331 & 0.33493 & 0.330558 & 0.289567 & 0.282766 \\ 
    60    & 0.412342 & 0.42981 & 0.453336 & 0.509178 & 0.854843 & 0.838063 & 0.923695 & 0.909187 & 0.914349 & 0.905471 & 0.950281 & 0.944189 & 0.762977 & 0.855222 & 0.8815 & 1.036068 & 332.6913 & 234.159 & 773.378 & 1811.135 & 0.670957 & 0.664425 & 0.697778 & 0.693894 & 0.340567 & 0.329467 & 0.295802 & 0.282824 \\ 
    72    & 0.425745 & 0.433164 & 0.454716 & 0.511242 & 0.860383 & 0.835044 & 0.916119 & 0.912341 & 0.918101 & 0.904226 & 0.94783 & 0.94623 & 0.836273 & 0.869014 & 0.88688 & 1.042941 & 334.7748 & 308.5081 & 929.3249 & 2321.105 & 0.673956 & 0.66326 & 0.695989 & 0.694682 &       &       &       &  \\ 
    168   & 0.433829 & 0.459476 & 0.465204 & 0.518881 & 0.914105 & 0.895081 & 0.974607 & 0.987383 & 0.945799 & 0.936521 & 0.975565 & 0.982565 & 0.843701 & 0.990876 & 0.883375 & 1.033184 & 277.3096 & 203.4026 & 1824.682 & 3049.109 & 0.691078 & 0.684312 & 0.71245 & 0.718241 & 0.323172 & 0.31895 & 0.295266 & 0.281929 \\ 
    336   & 0.438291 & 0.481645 & 0.481418 & 0.516939 & 0.971715 & 0.93894 & 0.997172 & 0.975083 & 0.978938 & 0.962202 & 0.99248 & 0.980915 & 0.785174 & 1.024626 & 0.911371 & 1.037195 & 203.4478 & 213.3468 & 240.1216 & 308.9575 & 0.714823 & 0.702821 & 0.724202 & 0.716339 &       &       &       &  \\ 
          &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\ 
          & 6.82\% &       & 7.51\% &       & -3.21\% &       & -3.06\% &       & -1.53\% &       & -1.45\% &       & 11.63\% &       & 9.74\% &       & -49.70\% &       & -55.26\% &       & -1.44\% &       & -1.41\% &       & 2.55\% &       & 1.08\% &  \\ 
          & 5.19\% &       & 9.33\% &       & -1.69\% &       & -1.62\% &       & -0.81\% &       & -0.83\% &       & 5.49\% &       & 12.55\% &       & 75.08\% &       & 39.81\% &       & -0.81\% &       & -0.86\% &       & 1.20\% &       & -1.45\% &  \\ 
          & 5.02\% &       & 10.08\% &       & -2.26\% &       & -1.24\% &       & -1.09\% &       & -0.60\% &       & 8.99\% &       & 13.60\% &       & -89.69\% &       & 37.78\% &       & -1.08\% &       & -0.53\% &       & 0.98\% &       & -2.21\% &  \\ 
          & 4.46\% &       & 10.84\% &       & -1.46\% &       & 0.02\% &       & -0.68\% &       & 0.08\% &       & 1.71\% &       & 13.97\% &       & -106.80\% &       & 18.62\% &       & -0.65\% &       & 0.20\% &       & -0.32\% &       & 0.35\% &  \\ 
          & 8.77\% &       & 11.60\% &       & -2.16\% &       & 1.92\% &       & -1.04\% &       & 1.00\% &       & 20.21\% &       & 14.19\% &       & 14.56\% &       & 69.70\% &       & -1.03\% &       & 1.07\% &       & 1.44\% &       & -2.57\% &  \\ 
          & 6.00\% &       & 10.36\% &       & -2.32\% &       & -0.58\% &       & -1.11\% &       & -0.29\% &       & 9.43\% &       & 13.78\% &       & 46.89\% &       & 60.04\% &       & -1.09\% &       & -0.22\% &       & -1.32\% &       & -2.41\% &  \\ 
          & 4.06\% &       & 10.97\% &       & -2.00\% &       & -1.60\% &       & -0.98\% &       & -0.65\% &       & 10.79\% &       & 14.92\% &       & -42.08\% &       & 57.30\% &       & -0.98\% &       & -0.56\% &       & -3.37\% &       & -4.59\% &  \\ 
          & 1.71\% &       & 11.06\% &       & -3.03\% &       & -0.41\% &       & -1.53\% &       & -0.17\% &       & 3.77\% &       & 14.96\% &       & -8.51\% &       & 59.96\% &       & -1.61\% &       & -0.19\% &       & \#DIV/0! &       & \#DIV/0! &  \\ 
          & 5.58\% &       & 10.34\% &       & -2.13\% &       & 1.29\% &       & -0.99\% &       & 0.71\% &       & 14.85\% &       & 14.50\% &       & -36.34\% &       & 40.16\% &       & -0.99\% &       & 0.81\% &       & -1.32\% &       & -4.73\% &  \\ 
          & 9.00\% &       & 6.87\% &       & -3.49\% &       & -2.27\% &       & -1.74\% &       & -1.18\% &       & 23.37\% &       & 12.13\% &       & 4.64\% &       & 22.28\% &       & -1.71\% &       & -1.10\% &       & \#DIV/0! &       & \#DIV/0! &  \\ 
    \end{tabular}%
}
\caption{}
\label{tab:addlabel}
  %

==> src/table/muti_horizon_without_msp.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{ABLATION WITHOUT MSP: We conduct it on Ampds2 with HORIZON [1,6,12,24,36,48,60,72,168,336]}
    \begin{tabular}{c||ccrrcc}
    \toprule
    \multicolumn{1}{l}{Method} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{w/o MSP} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{1}{l}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} \\
    \midrule
    \midrule
    1     & 0.440  & 0.884  & 0.406  & 0.800  & \textbf{0.397 } & \textbf{0.775 } \\
    6     & 0.479  & 0.992  & 0.435  & 0.842  & \textbf{0.435 } & \textbf{0.850 } \\
    12    & 0.494  & 1.015  & 0.460  & 0.924  & \textbf{0.445 } & \textbf{0.869 } \\
    24    & 0.490  & 1.019  & 0.450  & 0.892  & \textbf{0.448 } & \textbf{0.874 } \\
    36    & 0.496  & 1.009  & 0.456  & 0.903  & \textbf{0.448 } & \textbf{0.882 } \\
    48    & 0.497  & 1.021  & 0.452  & 0.885  & \textbf{0.450 } & \textbf{0.881 } \\
    60    & 0.495  & 1.018  & 0.457  & 0.893  & \textbf{0.445 } & \textbf{0.863 } \\
    72    & 0.500  & 1.021  & \textbf{0.453 } & \textbf{0.903 } & 0.457  & 0.907  \\
    168   & 0.506  & 1.024  & \textbf{0.463 } & \textbf{0.889 } & 0.470  & 0.901  \\
    336   & 0.514  & 1.049  & 0.485  & 0.930  & \textbf{0.472 } & \textbf{0.896 } \\
    \bottomrule
    \end{tabular}%
  \label{tab:muti_horizon_without_msp}%
\end{table}%


==> src/table/muti_horizon_without_response.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{ABLATION WITHOUT Response loss: We conduct it on Ampds2 with HORIZON [1,6,12,24,36,48,60,72,168,336]}
    \begin{tabular}{c||cccccc}
    \toprule
    \multicolumn{1}{c}{Method} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{w/o response} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{1}{c}{Metric} & MAE   & MAPE` & MAE   & MAPE` & MAE   & MAPE` \\
    \midrule
    \midrule
    1     & 0.440  & 0.884  & 0.490  & 1.029  & \textbf{0.397 } & \textbf{0.775 } \\
    6     & 0.479  & 0.992  & 0.495  & 1.013  & \textbf{0.435 } & \textbf{0.850 } \\
    12    & 0.494  & 1.015  & 0.506  & 1.025  & \textbf{0.445 } & \textbf{0.869 } \\
    24    & 0.490  & 1.019  & 0.502  & 1.039  & \textbf{0.448 } & \textbf{0.874 } \\
    36    & 0.496  & 1.009  & 0.518  & 1.036  & \textbf{0.448 } & \textbf{0.882 } \\
    48    & 0.497  & 1.021  & 0.514  & 1.066  & \textbf{0.450 } & \textbf{0.881 } \\
    60    & 0.495  & 1.018  & 0.521  & 1.063  & \textbf{0.445 } & \textbf{0.863 } \\
    72    & 0.500  & 1.021  & 0.515  & 1.049  & \textbf{0.457 } & \textbf{0.907 } \\
    168   & 0.506  & 1.024  & 0.536  & 1.088  & \textbf{0.470 } & \textbf{0.901 } \\
    336   & 0.514  & 1.049  & 0.547  & 1.075  & \textbf{0.472 } & \textbf{0.896 } \\
    \bottomrule
    \end{tabular}%
  \label{tab:ABLATION WITHOUT Response loss}%
\end{table}%


==> src/table/rlf_compare.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{COMPARISON OF FORECASTING ERRORS BETWEEN THE Load Forecasting \\
  Methods AND OUR METHOD}
    \begin{tabular}{cc||cccccccc}
    \toprule
    \multicolumn{2}{c}{Model} & \multicolumn{2}{c}{mtl-gru} & \multicolumn{2}{c}{+ours} & \multicolumn{2}{c}{vae} & \multicolumn{2}{c}{+ours} \\
    \midrule
    \multicolumn{2}{c}{Metric} & mae   & mape  & mae   & mape  & mae   & mape  & mae   & mape \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}}} & 1     & 0.531  & 0.958  & \textbf{0.513 } & \textbf{0.848 } & 0.680  & 1.181  & \textbf{0.654 } & \textbf{1.021 } \\
    \multicolumn{1}{c|}{} & 6     & 0.601  & 1.095  & \textbf{0.559 } & \textbf{0.913 } & 0.659  & 1.181  & \textbf{0.654 } & \textbf{1.069 } \\
    \multicolumn{1}{c|}{} & 12    & 0.633  & 1.158  & \textbf{0.562 } & \textbf{0.910 } & 0.706  & 1.260  & \textbf{0.664 } & \textbf{1.000 } \\
    \multicolumn{1}{c|}{} & 24    & 0.627  & 1.145  & \textbf{0.611 } & \textbf{1.024 } & 0.681  & 1.181  & \textbf{0.677 } & \textbf{1.058 } \\
    \multicolumn{1}{c|}{} & 36    & 0.622  & 1.140  & \textbf{0.595 } & \textbf{0.976 } & 0.700  & 1.181  & \textbf{0.654 } & \textbf{1.005 } \\
    \multicolumn{1}{c|}{} & 48    & 0.641  & 1.171  & \textbf{0.602 } & \textbf{0.995 } & 0.735  & 1.293  & \textbf{0.697 } & \textbf{1.009 } \\
    \multicolumn{1}{c|}{} & 60    & 0.628  & 1.170  & \textbf{0.608 } & \textbf{0.996 } & 0.702  & 1.204  & \textbf{0.664 } & \textbf{0.993 } \\
    \multicolumn{1}{c|}{} & 72    & 0.650  & 1.198  & \textbf{0.610 } & \textbf{1.012 } & 0.722  & 1.201  & \textbf{0.670 } & \textbf{1.009 } \\
    \multicolumn{1}{c|}{} & 168   & 0.664  & 1.224  & \textbf{0.604 } & \textbf{0.983 } & 0.742  & 1.514  & \textbf{0.660 } & \textbf{1.019 } \\
    \multicolumn{1}{c|}{} & 336   & 0.734  & 1.290  & \textbf{0.656 } & \textbf{1.031 } & 0.721  & 1.302  & \textbf{0.697 } & \textbf{1.015 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}}} & 1     & 0.427  & 0.994  & \textbf{0.411 } & \textbf{0.940 } & 0.506  & 1.102  & \textbf{0.494 } & \textbf{1.034 } \\
    \multicolumn{1}{c|}{} & 6     & 0.510  & 1.176  & \textbf{0.474 } & \textbf{1.063 } & \textbf{0.507 } & 1.065  & 0.507  & \textbf{1.057 } \\
    \multicolumn{1}{c|}{} & 12    & 0.530  & 1.229  & \textbf{0.484 } & \textbf{1.058 } & 0.521  & 1.179  & \textbf{0.505 } & \textbf{1.073 } \\
    \multicolumn{1}{c|}{} & 24    & 0.538  & 1.226  & \textbf{0.493 } & \textbf{1.089 } & 0.529  & 1.152  & \textbf{0.510 } & \textbf{1.044 } \\
    \multicolumn{1}{c|}{} & 36    & 0.547  & 1.212  & \textbf{0.496 } & \textbf{1.104 } & 0.532  & 1.175  & \textbf{0.505 } & \textbf{1.050 } \\
    \multicolumn{1}{c|}{} & 48    & 0.532  & 1.231  & \textbf{0.487 } & \textbf{1.115 } & 0.510  & 1.154  & \textbf{0.497 } & \textbf{1.088 } \\
    \multicolumn{1}{c|}{} & 60    & 0.535  & 1.245  & \textbf{0.490 } & \textbf{1.117 } & 0.515  & 1.157  & \textbf{0.489 } & \textbf{1.067 } \\
    \multicolumn{1}{c|}{} & 72    & 0.534  & 1.258  & \textbf{0.491 } & \textbf{1.134 } & 0.522  & 1.165  & \textbf{0.491 } & \textbf{1.056 } \\
    \multicolumn{1}{c|}{} & 168   & 0.528  & 1.277  & \textbf{0.483 } & \textbf{1.075 } & 0.501  & 1.146  & \textbf{0.474 } & \textbf{1.021 } \\
    \multicolumn{1}{c|}{} & 336   & 0.519  & 1.224  & \textbf{0.481 } & \textbf{1.086 } & 0.526  & 1.501  & \textbf{0.468 } & \textbf{1.009 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Umass3\end{sideways}}} & 1     & 0.410  & 0.890  & \textbf{0.362 } & \textbf{0.703 } & 0.472  & 0.965  & \textbf{0.457 } & \textbf{0.873 } \\
    \multicolumn{1}{c|}{} & 6     & 0.489  & 1.051  & \textbf{0.435 } & \textbf{0.887 } & 0.519  & 1.065  & \textbf{0.481 } & \textbf{0.963 } \\
    \multicolumn{1}{c|}{} & 12    & 0.515  & 1.120  & \textbf{0.454 } & \textbf{0.883 } & 0.541  & 1.156  & \textbf{0.481 } & \textbf{1.009 } \\
    \multicolumn{1}{c|}{} & 24    & 0.508  & 1.070  & \textbf{0.467 } & \textbf{0.923 } & 0.555  & 1.243  & \textbf{0.477 } & \textbf{0.983 } \\
    \multicolumn{1}{c|}{} & 36    & 0.517  & 1.105  & \textbf{0.467 } & \textbf{0.918 } & 0.552  & 1.193  & \textbf{0.469 } & \textbf{0.973 } \\
    \multicolumn{1}{c|}{} & 48    & 0.523  & 1.143  & \textbf{0.463 } & \textbf{0.928 } & 0.537  & 1.155  & \textbf{0.481 } & \textbf{0.983 } \\
    \multicolumn{1}{c|}{} & 60    & 0.521  & 1.136  & \textbf{0.465 } & \textbf{0.919 } & 0.555  & 1.406  & \textbf{0.464 } & \textbf{0.937 } \\
    \multicolumn{1}{c|}{} & 72    & 0.528  & 1.161  & \textbf{0.468 } & \textbf{0.921 } & 0.564  & 1.269  & \textbf{0.480 } & \textbf{0.952 } \\
    \multicolumn{1}{c|}{} & 168   & 0.540  & 1.193  & \textbf{0.491 } & \textbf{0.935 } & 0.527  & 1.166  & \textbf{0.457 } & \textbf{0.892 } \\
    \multicolumn{1}{c|}{} & 336   & 0.556  & 1.213  & \textbf{0.488 } & \textbf{0.938 } & 0.599  & 1.680  & \textbf{0.476 } & \textbf{0.916 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Umass4\end{sideways}}} & 1     & 0.328  & 0.918  & \textbf{0.290 } & \textbf{0.836 } & 0.458  & 1.177  & \textbf{0.401 } & \textbf{1.060 } \\
    \multicolumn{1}{c|}{} & 6     & 0.413  & 1.107  & \textbf{0.377 } & \textbf{1.022 } & 0.464  & 1.289  & \textbf{0.441 } & \textbf{1.243 } \\
    \multicolumn{1}{c|}{} & 12    & 0.445  & 1.162  & \textbf{0.433 } & \textbf{1.115 } & 0.437  & 1.208  & \textbf{0.423 } & \textbf{1.155 } \\
    \multicolumn{1}{c|}{} & 24    & 0.468  & 1.196  & \textbf{0.407 } & \textbf{1.104 } & 0.475  & 1.605  & \textbf{0.402 } & \textbf{1.217 } \\
    \multicolumn{1}{c|}{} & 36    & 0.446  & 1.264  & \textbf{0.385 } & \textbf{1.116 } & 0.457  & 1.398  & \textbf{0.398 } & \textbf{1.143 } \\
    \multicolumn{1}{c|}{} & 48    & 0.516  & 1.271  & \textbf{0.432 } & \textbf{1.154 } & 0.456  & 1.626  & \textbf{0.403 } & \textbf{1.201 } \\
    \multicolumn{1}{c|}{} & 60    & 0.453  & 1.258  & \textbf{0.441 } & \textbf{1.192 } & 0.463  & 1.577  & \textbf{0.405 } & \textbf{1.172 } \\
    \multicolumn{1}{c|}{} & 72    & 0.464  & 1.279  & \textbf{0.411 } & \textbf{1.174 } & 0.454  & 1.667  & \textbf{0.412 } & \textbf{1.240 } \\
    \multicolumn{1}{c|}{} & 168   & 0.485  & 1.350  & \textbf{0.463 } & \textbf{1.143 } & 0.477  & 1.628  & \textbf{0.420 } & \textbf{1.127 } \\
    \multicolumn{1}{c|}{} & 336   & \textbf{0.446 } & 1.325  & 0.448  & \textbf{1.143 } & 0.465  & 1.506  & \textbf{0.395 } & \textbf{1.141 } \\
    \midrule
    \multicolumn{2}{c||}{Avg \% Imp} & /     & /     & \textbf{8.31\%} & \textbf{13.72\%} & /     & /     & \textbf{8.22\%} & \textbf{17.20\%} \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%


==> src/table/table.tex <==
% % Tble generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{c|c||rrrr|rrrr|rrrr}
%     \toprule
%     \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TS-mixer} & \multicolumn{2}{c}{ +ours} \\
%     % \midrule
%     \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%     \cmidrule(r){9-10} \cmidrule(r){11-12}  \cmidrule(r){13-14}
%     \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
%     \midrule
%     \midrule
%     \multirow{10}[2]{*}{Ampds2} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{UK-DALEh1} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{UK-DALEh2} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{UK-DALEh4} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{UK-DALEh5} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%


% % Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table*}[h]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{c|c||rrrr|rrrr|rrrr}
%     \toprule
%     \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TS-mixer} & \multicolumn{2}{c}{ +ours} \\
%     % \midrule
%     \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%     \cmidrule(r){9-10} \cmidrule(r){11-12}  \cmidrule(r){13-14}
%     \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
%     \midrule
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh2\end{sideways}} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh4\end{sideways}} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh5\end{sideways}} & 1     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 6     &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 12    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 24    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 36    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 48    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 60    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 72    &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 168   &       &       &       &       &       &       &       &       &       &       &       &  \\
%           & 336   &       &       &       &       &       &       &       &       &       &       &       &  \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{c|c||cccccccccccc}
%     \toprule
%     \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TS-mixer} & \multicolumn{2}{c}{ +ours} \\
% %     % \midrule
%     \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
%     \cmidrule(r){9-10} \cmidrule(r){11-12}  \cmidrule(r){13-14}
%     \multicolumn{2}{c}{Metric} & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE \\
%     \midrule
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}} & 1     & 0.379  & 0.744  & \textbf{0.360 } & \textbf{0.700 } & 0.440  & 0.884  & \textbf{0.397 } & \textbf{0.775 } & 0.387  & 0.753  & \textbf{0.383 } & \textbf{0.692 } \\
%           & 6     & 0.420  & 0.841  & \textbf{0.396 } & \textbf{0.799 } & 0.479  & 0.992  & \textbf{0.435 } & \textbf{0.850 } & 0.425  & 0.884  & \textbf{0.396 } & \textbf{0.745 } \\
%           & 12    & 0.435  & 0.887  & \textbf{0.407 } & \textbf{0.799 } & 0.494  & 1.015  & \textbf{0.445 } & \textbf{0.869 } & 0.434  & 0.924  & \textbf{0.401 } & \textbf{0.757 } \\
%           & 24    & 0.429  & 0.806  & \textbf{0.424 } & 0.908  & 0.490  & 1.019  & \textbf{0.448 } & \textbf{0.874 } & 0.435  & 0.922  & \textbf{0.404 } & \textbf{0.760 } \\
%           & 36    & 0.449  & 0.939  & \textbf{0.419 } & \textbf{0.875 } & 0.496  & 1.009  & \textbf{0.448 } & \textbf{0.882 } & 0.438  & 0.919  & \textbf{0.408 } & \textbf{0.762 } \\
%           & 48    & 0.446  & 0.925  & \textbf{0.417 } & \textbf{0.817 } & 0.497  & 1.021  & \textbf{0.450 } & \textbf{0.881 } & 0.440  & 0.922  & \textbf{0.408 } & \textbf{0.762 } \\
%           & 60    & 0.430  & 0.855  & \textbf{0.412 } & \textbf{0.778 } & 0.495  & 1.018  & \textbf{0.445 } & \textbf{0.863 } & 0.441  & 0.930  & \textbf{0.410 } & \textbf{0.758 } \\
%           & 72    & 0.433  & 0.869  & \textbf{0.417 } & \textbf{0.786 } & 0.500  & 1.021  & \textbf{0.457 } & \textbf{0.907 } & 0.444  & 0.932  & \textbf{0.410 } & \textbf{0.764 } \\
%           & 168   & 0.454  & 0.878  & \textbf{0.446 } & 0.938  & 0.506  & 1.024  & \textbf{0.470 } & \textbf{0.901 } & 0.456  & 0.952  & \textbf{0.426 } & \textbf{0.796 } \\
%           & 336   & 0.482  & 1.025  & \textbf{0.439 } & \textbf{0.811 } & 0.514  & 1.049  & \textbf{0.472 } & \textbf{0.896 } & 0.471  & 0.973  & \textbf{0.442 } & \textbf{0.840 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}} & 1     & 0.377  & 0.843  & \textbf{0.347 } & \textbf{0.742 } & 0.488  & 0.958  & \textbf{0.460 } & \textbf{0.918 } & 0.362  & 0.692  & \textbf{0.369 } & 0.737  \\
%           & 6     & 0.417  & 0.782  & \textbf{0.401 } & \textbf{0.727 } & 0.561  & 1.062  & \textbf{0.536 } & \textbf{1.039 } & 0.441  & 0.847  & \textbf{0.427 } & \textbf{0.814 } \\
%           & 12    & 0.467  & 0.950  & \textbf{0.455 } & \textbf{0.922 } & 0.587  & 1.080  & \textbf{0.565 } & \textbf{1.049 } & 0.458  & 0.889  & \textbf{0.434 } & \textbf{0.827 } \\
%           & 24    & 0.471  & 0.934  & 0.474  & 0.994  & 0.600  & 1.104  & \textbf{0.562 } & \textbf{1.081 } & 0.470  & 0.910  & \textbf{0.444 } & \textbf{0.841 } \\
%           & 36    & 0.466  & 0.893  & \textbf{0.459 } & \textbf{0.851 } & 0.610  & 1.138  & \textbf{0.556 } & \textbf{1.071 } & 0.482  & 0.926  & \textbf{0.453 } & \textbf{0.850 } \\
%           & 48    & 0.482  & 0.988  & \textbf{0.449 } & \textbf{0.904 } & 0.595  & 1.114  & \textbf{0.547 } & \textbf{1.071 } & 0.465  & 0.922  & \textbf{0.444 } & \textbf{0.857 } \\
%           & 60    & 0.486  & 1.008  & \textbf{0.470 } & \textbf{0.974 } & 0.591  & 1.139  & \textbf{0.548 } & \textbf{1.076 } & 0.467  & 0.923  & \textbf{0.447 } & \textbf{0.856 } \\
%           & 72    & 0.482  & 0.993  & \textbf{0.474 } & \textbf{0.944 } & 0.589  & 1.129  & \textbf{0.540 } & \textbf{1.068 } & 0.471  & 0.934  & \textbf{0.456 } & \textbf{0.911 } \\
%           & 168   & 0.491  & 1.043  & \textbf{0.462 } & \textbf{0.938 } & 0.574  & 1.147  & \textbf{0.518 } & \textbf{1.060 } & 0.471  & 0.949  & \textbf{0.445 } & \textbf{0.861 } \\
%           & 336   & 0.481  & 1.052  & \textbf{0.450 } & \textbf{0.895 } & 0.567  & 1.141  & \textbf{0.515 } & \textbf{1.062 } & 0.468  & 0.951  & \textbf{0.447 } & \textbf{0.878 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh2\end{sideways}} & 1     & 1.022  & 0.965  & 1.046  & \textbf{0.888 } & 0.403  & 0.804  & \textbf{0.432 } & 0.821  & 0.430  & 0.741  & \textbf{0.390 } & \textbf{0.710 } \\
%           & 6     & 0.809  & 1.007  & 0.836  & \textbf{0.816 } & 0.695  & 0.993  & \textbf{0.726 } & \textbf{0.953 } & 0.543  & 0.861  & \textbf{0.459 } & \textbf{0.816 } \\
%           & 12    & 0.917  & 0.917  & \textbf{0.867 } & \textbf{0.878 } & 0.693  & 1.061  & \textbf{0.657 } & \textbf{1.030 } & 0.645  & 0.992  & \textbf{0.590 } & \textbf{0.961 } \\
%           & 24    & 0.981  & 0.974  & \textbf{0.919 } & \textbf{0.922 } & 0.757  & 1.030  & \textbf{0.653 } & \textbf{1.008 } & 0.671  & 1.030  & \textbf{0.616 } & \textbf{0.970 } \\
%           & 36    & 1.042  & 0.970  & \textbf{1.019 } & 0.995  & 0.697  & 1.054  & \textbf{0.691 } & \textbf{1.047 } & 0.785  & 1.072  & \textbf{0.680 } & \textbf{1.007 } \\
%           & 48    & 1.050  & 0.974  & 1.134  & 1.015  & 0.750  & 1.066  & \textbf{0.723 } & \textbf{1.050 } & 0.900  & 1.161  & \textbf{0.743 } & \textbf{1.003 } \\
%           & 60    & 1.051  & 1.029  & \textbf{1.039 } & 1.037  & 0.860  & 1.107  & \textbf{0.751 } & \textbf{1.051 } & 0.838  & 1.086  & \textbf{0.813 } & \textbf{1.043 } \\
%           & 72    & 1.159  & 1.101  & 1.216  & \textbf{1.051 } & 1.031  & 1.137  & \textbf{0.942 } & \textbf{1.110 } & 0.887  & 1.123  & \textbf{0.825 } & \textbf{1.105 } \\
%           & 168   & 1.308  & 1.181  & \textbf{1.281 } & \textbf{1.165 } & 1.304  & 1.264  & \textbf{1.137 } & \textbf{1.199 } & 1.264  & 1.272  & \textbf{1.150 } & \textbf{1.210 } \\
%           & 336   & 1.918  & 1.298  & \textbf{1.891 } & \textbf{1.253 } & 1.654  & 1.378  & \textbf{1.644 } & \textbf{1.356 } & 1.763  & 1.378  & \textbf{1.710 } & \textbf{1.374 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh4\end{sideways}} & 1     & 0.486  & 1.092  & \textbf{0.477 } & \textbf{0.987 } & 0.454  & 1.086  & \textbf{0.497 } & \textbf{1.076 } & 0.412  & 0.926  & \textbf{0.410 } & 0.942  \\
%           & 6     & 0.572  & 0.950  & 0.581  & \textbf{0.948 } & 0.515  & 1.142  & \textbf{0.485 } & \textbf{1.109 } & 0.462  & 1.107  & \textbf{0.437 } & \textbf{0.973 } \\
%           & 12    & 0.608  & 1.130  & \textbf{0.552 } & 1.139  & 0.541  & 1.174  & \textbf{0.569 } & 1.184  & 0.467  & 1.085  & \textbf{0.449 } & \textbf{1.024 } \\
%           & 24    & 0.591  & 1.174  & \textbf{0.557 } & \textbf{1.079 } & 0.529  & 1.190  & \textbf{0.543 } & \textbf{1.143 } & 0.482  & 1.145  & \textbf{0.457 } & \textbf{1.016 } \\
%           & 36    & 0.603  & 1.148  & \textbf{0.599 } & \textbf{1.085 } & 0.553  & 1.204  & \textbf{0.543 } & \textbf{1.180 } & 0.488  & 1.122  & \textbf{0.478 } & \textbf{1.097 } \\
%           & 48    & 0.545  & 1.048  & 0.584  & 1.150  & 0.556  & 1.173  & \textbf{0.518 } & \textbf{1.125 } & 0.489  & 1.136  & \textbf{0.479 } & \textbf{1.109 } \\
%           & 60    & 0.606  & 1.102  & \textbf{0.605 } & 1.134  & 0.547  & 1.170  & \textbf{0.543 } & 1.171  & 0.493  & 1.127  & \textbf{0.485 } & \textbf{1.108 } \\
%           & 72    & 0.605  & 1.081  & 0.607  & 1.129  & 0.581  & 1.225  & \textbf{0.552 } & \textbf{1.162 } & 0.499  & 1.147  & \textbf{0.494 } & \textbf{1.123 } \\
%           & 168   & 0.582  & 1.098  & \textbf{0.577 } & 1.151  & 0.616  & 1.208  & \textbf{0.644 } & 1.223  & 0.517  & 1.124  & \textbf{0.515 } & \textbf{1.122 } \\
%           & 336   & 0.604  & 1.106  & \textbf{0.601 } & \textbf{0.991 } & 0.667  & 1.302  & \textbf{0.636 } & \textbf{1.205 } & 0.577  & 1.158  & \textbf{0.569 } & \textbf{1.152 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UK-DALEh5\end{sideways}} & 1     & 0.627  & 1.095  & \textbf{0.601 } & \textbf{0.878 } & 0.744  & 1.005  & \textbf{0.617 } & \textbf{0.962 } & 0.396  & 0.818  & \textbf{0.374 } & \textbf{0.781 } \\
%           & 6     & 0.696  & 0.999  & \textbf{0.580 } & \textbf{0.814 } & 0.780  & 1.106  & \textbf{0.914 } & \textbf{1.071 } & 0.473  & 0.903  & \textbf{0.453 } & \textbf{0.841 } \\
%           & 12    & 0.675  & 1.007  & 0.710  & \textbf{0.850 } & 1.014  & 1.139  & \textbf{0.923 } & \textbf{1.070 } & 0.487  & 0.923  & \textbf{0.442 } & \textbf{0.833 } \\
%           & 24    & 0.800  & 0.918  & \textbf{0.765 } & \textbf{0.917 } & 1.135  & 1.148  & \textbf{1.084 } & \textbf{1.119 } & 0.580  & 0.963  & \textbf{0.538 } & \textbf{0.877 } \\
%           & 36    & 0.778  & 1.055  & \textbf{0.738 } & \textbf{0.974 } & 1.511  & 1.188  & \textbf{1.255 } & \textbf{1.183 } & 0.660  & 0.993  & \textbf{0.612 } & \textbf{0.959 } \\
%           & 48    & 0.746  & 0.991  & \textbf{0.738 } & 1.021  & 1.702  & 1.220  & \textbf{1.484 } & \textbf{1.174 } & 0.685  & 1.007  & \textbf{0.627 } & \textbf{0.937 } \\
%           & 60    & 0.755  & 1.000  & 0.788  & \textbf{0.990 } & 1.594  & 1.212  & \textbf{1.545 } & \textbf{1.180 } & 0.698  & 1.019  & \textbf{0.656 } & \textbf{0.959 } \\
%           & 72    & 0.739  & 0.933  & \textbf{0.683 } & 1.014  & 1.160  & 1.168  & \textbf{1.393 } & 1.205  & 0.724  & 1.040  & \textbf{0.605 } & \textbf{0.929 } \\
%           & 168   & 0.756  & 0.989  & \textbf{0.733 } & 0.990  & 2.131  & 1.284  & \textbf{1.956 } & \textbf{1.240 } & 0.756  & 1.063  & \textbf{0.725 } & \textbf{0.998 } \\
%           & 336   & 0.868  & 1.049  & \textbf{0.788 } & \textbf{1.006 } & 1.307  & 1.192  & \textbf{1.516 } & 1.201  & 0.901  & 1.128  & \textbf{0.856 } & \textbf{1.079 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UMASS1\end{sideways}} & 1     & 0.807  & 0.785  & \textbf{0.673 } & \textbf{0.615 } & 0.920  & 0.927  & \textbf{0.854 } & \textbf{0.856 } & 0.606  & 0.667  & \textbf{0.589 } & \textbf{0.595 } \\
%           & 6     & 0.821  & 0.764  & \textbf{0.715 } & \textbf{0.662 } & 1.044  & 0.978  & \textbf{0.980 } & \textbf{0.926 } & 0.719  & 0.802  & \textbf{0.712 } & \textbf{0.767 } \\
%           & 12    & 0.809  & 0.738  & \textbf{0.735 } & \textbf{0.711 } & 1.108  & 0.999  & \textbf{1.033 } & \textbf{0.949 } & 0.710  & 0.780  & \textbf{0.712 } & \textbf{0.757 } \\
%           & 24    & 0.832  & 0.743  & 0.846  & 0.757  & 1.076  & 1.004  & \textbf{0.988 } & \textbf{0.946 } & 0.725  & 0.796  & \textbf{0.685 } & \textbf{0.718 } \\
%           & 36    & 0.928  & 0.868  & \textbf{0.811 } & \textbf{0.839 } & 1.097  & 1.017  & \textbf{1.033 } & \textbf{0.949 } & 0.730  & 0.801  & \textbf{0.706 } & \textbf{0.741 } \\
%           & 48    & 1.024  & 0.981  & \textbf{0.836 } & \textbf{0.802 } & 1.095  & 1.021  & \textbf{1.048 } & \textbf{0.968 } & 0.738  & 0.804  & \textbf{0.737 } & \textbf{0.769 } \\
%           & 60    & 0.794  & 0.778  & \textbf{0.782 } & 0.790  & 1.078  & 1.011  & \textbf{1.051 } & \textbf{0.984 } & 0.748  & 0.817  & \textbf{0.705 } & \textbf{0.727 } \\
%           & 72    & 0.900  & 0.948  & \textbf{0.736 } & \textbf{0.671 } & 1.128  & 1.017  & \textbf{1.101 } & \textbf{1.002 } & 0.749  & 0.814  & \textbf{0.712 } & \textbf{0.745 } \\
%           & 168   & 0.866  & 0.896  & \textbf{0.764 } & \textbf{0.763 } & 1.156  & 1.029  & \textbf{1.102 } & \textbf{0.990 } & 0.770  & 0.828  & \textbf{0.750 } & \textbf{0.771 } \\
%           & 336   & 0.948  & 1.019  & \textbf{0.822 } & \textbf{0.783 } & 1.192  & 1.054  & \textbf{1.103 } & \textbf{1.001 } & 0.802  & 0.832  & \textbf{0.763 } & \textbf{0.774 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UMASS2\end{sideways}} & 1     & 0.950  & 0.586  & \textbf{0.930 } & 0.667  & 1.381  & 0.744  & \textbf{1.269 } & \textbf{0.705 } & 0.824  & 0.565  & \textbf{0.751 } & \textbf{0.510 } \\
%           & 6     & 1.051  & 0.712  & \textbf{0.906 } & \textbf{0.613 } & 1.498  & 0.787  & \textbf{1.444 } & \textbf{0.752 } & 0.945  & 0.630  & \textbf{0.860 } & \textbf{0.574 } \\
%           & 12    & 0.972  & 0.653  & \textbf{0.966 } & \textbf{0.644 } & 1.537  & 0.805  & \textbf{1.558 } & \textbf{0.793 } & 1.064  & 0.691  & \textbf{0.988 } & \textbf{0.647 } \\
%           & 24    & 1.162  & 0.708  & \textbf{1.038 } & \textbf{0.687 } & 1.661  & 0.844  & \textbf{1.514 } & \textbf{0.808 } & 1.029  & 0.698  & \textbf{0.932 } & \textbf{0.656 } \\
%           & 36    & 1.110  & 0.706  & \textbf{0.983 } & \textbf{0.651 } & 1.706  & 0.843  & \textbf{1.522 } & \textbf{0.807 } & 1.070  & 0.712  & \textbf{0.951 } & \textbf{0.650 } \\
%           & 48    & 1.193  & 0.795  & \textbf{0.972 } & \textbf{0.666 } & 1.741  & 0.866  & \textbf{1.561 } & \textbf{0.828 } & 1.031  & 0.703  & \textbf{0.934 } & \textbf{0.644 } \\
%           & 60    & 1.222  & 0.819  & \textbf{1.215 } & \textbf{0.788 } & 1.768  & 0.904  & \textbf{1.593 } & \textbf{0.838 } & 1.045  & 0.712  & \textbf{0.955 } & \textbf{0.655 } \\
%           & 72    & 1.103  & 0.777  & \textbf{1.087 } & \textbf{0.737 } & 1.909  & 0.914  & \textbf{1.729 } & \textbf{0.863 } & 1.059  & 0.730  & \textbf{0.951 } & \textbf{0.663 } \\
%           & 168   & 1.605  & 0.800  & \textbf{1.365 } & 0.837  & 1.788  & 0.869  & \textbf{1.619 } & \textbf{0.841 } & 1.061  & 0.738  & \textbf{0.964 } & \textbf{0.679 } \\
%           & 336   & 1.281  & 0.822  & \textbf{1.172 } & \textbf{0.755 } & 2.292  & 0.958  & \textbf{2.057 } & \textbf{0.910 } & 1.098  & 0.757  & \textbf{1.010 } & \textbf{0.683 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UMASS3\end{sideways}} & 1     & 0.401  & 0.883  & \textbf{0.380 } & \textbf{0.838 } & 0.490  & 1.032  & \textbf{0.439 } & \textbf{0.928 } & 0.426  & 0.901  & \textbf{0.399 } & \textbf{0.806 } \\
%           & 6     & 0.483  & 1.041  & \textbf{0.420 } & \textbf{0.857 } & 0.577  & 1.167  & \textbf{0.518 } & \textbf{1.067 } & 0.495  & 1.083  & \textbf{0.440 } & \textbf{0.931 } \\
%           & 12    & 0.497  & 1.042  & \textbf{0.430 } & \textbf{0.871 } & 0.603  & 1.213  & \textbf{0.514 } & \textbf{1.061 } & 0.487  & 1.046  & \textbf{0.435 } & \textbf{0.878 } \\
%           & 24    & 0.488  & 1.031  & \textbf{0.478 } & \textbf{1.025 } & 0.596  & 1.193  & \textbf{0.530 } & \textbf{1.079 } & 0.504  & 1.085  & \textbf{0.452 } & \textbf{0.950 } \\
%           & 36    & 0.487  & 1.027  & \textbf{0.450 } & \textbf{0.919 } & 0.603  & 1.200  & \textbf{0.524 } & \textbf{1.064 } & 0.501  & 1.087  & \textbf{0.440 } & \textbf{0.898 } \\
%           & 48    & 0.488  & 1.043  & \textbf{0.452 } & \textbf{0.908 } & 0.607  & 1.208  & \textbf{0.507 } & \textbf{1.060 } & 0.502  & 1.094  & \textbf{0.448 } & \textbf{0.924 } \\
%           & 60    & 0.481  & 0.996  & \textbf{0.456 } & \textbf{0.948 } & 0.605  & 1.223  & \textbf{0.533 } & \textbf{1.111 } & 0.513  & 1.120  & \textbf{0.460 } & \textbf{0.988 } \\
%           & 72    & 0.513  & 1.117  & \textbf{0.465 } & \textbf{0.912 } & 0.624  & 1.243  & \textbf{0.516 } & \textbf{1.089 } & 0.506  & 1.092  & \textbf{0.458 } & \textbf{0.963 } \\
%           & 168   & 0.504  & 1.089  & \textbf{0.465 } & \textbf{0.953 } & 0.613  & 1.226  & \textbf{0.516 } & \textbf{1.066 } & 0.513  & 1.130  & \textbf{0.458 } & \textbf{0.946 } \\
%           & 336   & 0.521  & 1.112  & \textbf{0.480 } & \textbf{0.976 } & 0.624  & 1.221  & \textbf{0.555 } & \textbf{1.080 } & 0.521  & 1.129  & \textbf{0.471 } & \textbf{0.975 } \\
%     \midrule
%     \multirow{10}[2]{*}{\begin{sideways}UMASS4\end{sideways}} & 1     & 0.255  & 0.654  & \textbf{0.206 } & \textbf{0.504 } & 0.354  & 0.719  & \textbf{0.322 } & \textbf{0.674 } & 0.222  & 0.548  & \textbf{0.205 } & \textbf{0.498 } \\
%           & 6     & 0.288  & 0.622  & \textbf{0.265 } & \textbf{0.561 } & 0.430  & 0.846  & \textbf{0.386 } & \textbf{0.773 } & 0.271  & 0.660  & \textbf{0.240 } & \textbf{0.580 } \\
%           & 12    & 0.288  & 0.696  & \textbf{0.287 } & \textbf{0.666 } & 0.466  & 0.869  & \textbf{0.430 } & \textbf{0.806 } & 0.270  & 0.648  & \textbf{0.254 } & \textbf{0.599 } \\
%           & 24    & 0.283  & 0.698  & \textbf{0.270 } & \textbf{0.659 } & 0.451  & 0.860  & \textbf{0.429 } & \textbf{0.817 } & 0.289  & 0.680  & \textbf{0.263 } & \textbf{0.621 } \\
%           & 36    & 0.341  & 0.828  & \textbf{0.286 } & \textbf{0.661 } & 0.519  & 0.892  & \textbf{0.442 } & \textbf{0.830 } & 0.304  & 0.723  & \textbf{0.276 } & \textbf{0.656 } \\
%           & 48    & 0.342  & 0.832  & \textbf{0.341 } & \textbf{0.801 } & 0.477  & 0.888  & \textbf{0.439 } & \textbf{0.837 } & 0.290  & 0.698  & \textbf{0.265 } & \textbf{0.641 } \\
%           & 60    & 0.323  & 0.738  & \textbf{0.303 } & \textbf{0.732 } & 0.522  & 0.899  & \textbf{0.492 } & \textbf{0.843 } & 0.283  & 0.693  & \textbf{0.257 } & \textbf{0.605 } \\
%           & 72    & 0.311  & 0.761  & \textbf{0.300 } & \textbf{0.665 } & 0.485  & 0.886  & \textbf{0.484 } & \textbf{0.830 } & 0.299  & 0.715  & \textbf{0.269 } & \textbf{0.638 } \\
%           & 168   & 0.375  & 0.897  & \textbf{0.353 } & \textbf{0.790 } & 0.527  & 0.915  & \textbf{0.484 } & \textbf{0.850 } & 0.316  & 0.732  & \textbf{0.292 } & \textbf{0.653 } \\
%           & 336   & 0.364  & 0.797  & \textbf{0.363 } & \textbf{0.755 } & 0.475  & 0.887  & \textbf{0.493 } & \textbf{0.858 } & 0.328  & 0.740  & \textbf{0.307 } & \textbf{0.670 } \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:addlabel}%
% \end{table}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Comparison of forecasting errors between the baselines and our method}
  \label{table:main result -0.1}
    \begin{tabular}{c|c||cccccccccccc}
    \toprule
    \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{ETSformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TSMixer} & \multicolumn{2}{c}{ +ours} \\
    % \midrule
    % %     % \midrule
    \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6} \cmidrule(r){7-8} 
    \cmidrule(r){9-10} \cmidrule(r){11-12}  \cmidrule(r){13-14}
    \multicolumn{2}{c}{Metric} & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE & MAE   & sMAPE \\
    \midrule
    \midrule
    \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{sMAPE} \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}}} & 1     & 0.379  & 0.744  & \textbf{0.360 } & \textbf{0.700 } & 0.440  & 0.884  & \textbf{0.397 } & \textbf{0.775 } & 0.387  & 0.753  & \textbf{0.383 } & \textbf{0.692 } \\
    \multicolumn{1}{c|}{} & 6     & 0.420  & 0.841  & \textbf{0.396 } & \textbf{0.799 } & 0.479  & 0.992  & \textbf{0.435 } & \textbf{0.850 } & 0.425  & 0.884  & \textbf{0.396 } & \textbf{0.745 } \\
    \multicolumn{1}{c|}{} & 12    & 0.435  & 0.887  & \textbf{0.407 } & \textbf{0.799 } & 0.494  & 1.015  & \textbf{0.445 } & \textbf{0.869 } & 0.434  & 0.924  & \textbf{0.401 } & \textbf{0.757 } \\
    \multicolumn{1}{c|}{} & 24    & 0.429  & \textbf{0.806 } & \textbf{0.424 } & 0.908  & 0.490  & 1.019  & \textbf{0.448 } & \textbf{0.874 } & 0.435  & 0.922  & \textbf{0.404 } & \textbf{0.760 } \\
    \multicolumn{1}{c|}{} & 36    & 0.449  & 0.939  & \textbf{0.419 } & \textbf{0.875 } & 0.496  & 1.009  & \textbf{0.448 } & \textbf{0.882 } & 0.438  & 0.919  & \textbf{0.408 } & \textbf{0.762 } \\
    \multicolumn{1}{c|}{} & 48    & 0.446  & 0.925  & \textbf{0.417 } & \textbf{0.817 } & 0.497  & 1.021  & \textbf{0.450 } & \textbf{0.881 } & 0.440  & 0.922  & \textbf{0.408 } & \textbf{0.762 } \\
    \multicolumn{1}{c|}{} & 60    & 0.430  & 0.855  & \textbf{0.412 } & \textbf{0.778 } & 0.495  & 1.018  & \textbf{0.445 } & \textbf{0.863 } & 0.441  & 0.930  & \textbf{0.410 } & \textbf{0.758 } \\
    \multicolumn{1}{c|}{} & 72    & 0.433  & 0.869  & \textbf{0.417 } & \textbf{0.786 } & 0.500  & 1.021  & \textbf{0.457 } & \textbf{0.907 } & 0.444  & 0.932  & \textbf{0.410 } & \textbf{0.764 } \\
    \multicolumn{1}{c|}{} & 168   & 0.454  & \textbf{0.878 } & \textbf{0.446 } & 0.938  & 0.506  & 1.024  & \textbf{0.470 } & \textbf{0.901 } & 0.456  & 0.952  & \textbf{0.426 } & \textbf{0.796 } \\
    \multicolumn{1}{c|}{} & 336   & 0.482  & 1.025  & \textbf{0.439 } & \textbf{0.811 } & 0.514  & 1.049  & \textbf{0.472 } & \textbf{0.896 } & 0.471  & 0.973  & \textbf{0.442 } & \textbf{0.840 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}UK-DALEh1\end{sideways}}} & 1     & 0.377  & 0.843  & \textbf{0.347 } & \textbf{0.742 } & 0.488  & 0.958  & \textbf{0.460 } & \textbf{0.918 } & \textbf{0.362 } & \textbf{0.692 } & 0.369  & 0.737  \\
    \multicolumn{1}{c|}{} & 6     & 0.417  & 0.782  & \textbf{0.401 } & \textbf{0.727 } & 0.561  & 1.062  & \textbf{0.536 } & \textbf{1.039 } & 0.441  & 0.847  & \textbf{0.427 } & \textbf{0.814 } \\
    \multicolumn{1}{c|}{} & 12    & 0.467  & 0.950  & \textbf{0.455 } & \textbf{0.922 } & 0.587  & 1.080  & \textbf{0.565 } & \textbf{1.049 } & 0.458  & 0.889  & \textbf{0.434 } & \textbf{0.827 } \\
    \multicolumn{1}{c|}{} & 24    & \textbf{0.471 } & \textbf{0.934 } & 0.474  & 0.994  & 0.600  & 1.104  & \textbf{0.562 } & \textbf{1.081 } & 0.470  & 0.910  & \textbf{0.444 } & \textbf{0.841 } \\
    \multicolumn{1}{c|}{} & 36    & 0.466  & 0.893  & \textbf{0.459 } & \textbf{0.851 } & 0.610  & 1.138  & \textbf{0.556 } & \textbf{1.071 } & 0.482  & 0.926  & \textbf{0.453 } & \textbf{0.850 } \\
    \multicolumn{1}{c|}{} & 48    & 0.482  & 0.988  & \textbf{0.449 } & \textbf{0.904 } & 0.595  & 1.114  & \textbf{0.547 } & \textbf{1.071 } & 0.465  & 0.922  & \textbf{0.444 } & \textbf{0.857 } \\
    \multicolumn{1}{c|}{} & 60    & 0.486  & 1.008  & \textbf{0.470 } & \textbf{0.974 } & 0.591  & 1.139  & \textbf{0.548 } & \textbf{1.076 } & 0.467  & 0.923  & \textbf{0.447 } & \textbf{0.856 } \\
    \multicolumn{1}{c|}{} & 72    & 0.482  & 0.993  & \textbf{0.474 } & \textbf{0.944 } & 0.589  & 1.129  & \textbf{0.540 } & \textbf{1.068 } & 0.471  & 0.934  & \textbf{0.456 } & \textbf{0.911 } \\
    \multicolumn{1}{c|}{} & 168   & 0.491  & 1.043  & \textbf{0.462 } & \textbf{0.938 } & 0.574  & 1.147  & \textbf{0.518 } & \textbf{1.060 } & 0.471  & 0.949  & \textbf{0.445 } & \textbf{0.861 } \\
    \multicolumn{1}{c|}{} & 336   & 0.481  & 1.052  & \textbf{0.450 } & \textbf{0.895 } & 0.567  & 1.141  & \textbf{0.515 } & \textbf{1.062 } & 0.468  & 0.951  & \textbf{0.447 } & \textbf{0.878 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Umass3\end{sideways}}} & 1     & 0.401  & 0.883  & \textbf{0.380 } & \textbf{0.838 } & 0.490  & 1.032  & \textbf{0.439 } & \textbf{0.928 } & 0.426  & 0.901  & \textbf{0.399 } & \textbf{0.806 } \\
    \multicolumn{1}{c|}{} & 6     & 0.483  & 1.041  & \textbf{0.420 } & \textbf{0.857 } & 0.577  & 1.167  & \textbf{0.518 } & \textbf{1.067 } & 0.495  & 1.083  & \textbf{0.440 } & \textbf{0.931 } \\
    \multicolumn{1}{c|}{} & 12    & 0.497  & 1.042  & \textbf{0.430 } & \textbf{0.871 } & 0.603  & 1.213  & \textbf{0.514 } & \textbf{1.061 } & 0.487  & 1.046  & \textbf{0.435 } & \textbf{0.878 } \\
    \multicolumn{1}{c|}{} & 24    & 0.488  & 1.031  & \textbf{0.478 } & \textbf{1.025 } & 0.596  & 1.193  & \textbf{0.530 } & \textbf{1.079 } & 0.504  & 1.085  & \textbf{0.452 } & \textbf{0.950 } \\
    \multicolumn{1}{c|}{} & 36    & 0.487  & 1.027  & \textbf{0.450 } & \textbf{0.919 } & 0.603  & 1.200  & \textbf{0.524 } & \textbf{1.064 } & 0.501  & 1.087  & \textbf{0.440 } & \textbf{0.898 } \\
    \multicolumn{1}{c|}{} & 48    & 0.488  & 1.043  & \textbf{0.452 } & \textbf{0.908 } & 0.607  & 1.208  & \textbf{0.507 } & \textbf{1.060 } & 0.502  & 1.094  & \textbf{0.448 } & \textbf{0.924 } \\
    \multicolumn{1}{c|}{} & 60    & 0.481  & 0.996  & \textbf{0.456 } & \textbf{0.948 } & 0.605  & 1.223  & \textbf{0.533 } & \textbf{1.111 } & 0.513  & 1.120  & \textbf{0.460 } & \textbf{0.988 } \\
    \multicolumn{1}{c|}{} & 72    & 0.513  & 1.117  & \textbf{0.465 } & \textbf{0.912 } & 0.624  & 1.243  & \textbf{0.516 } & \textbf{1.089 } & 0.506  & 1.092  & \textbf{0.458 } & \textbf{0.963 } \\
    \multicolumn{1}{c|}{} & 168   & 0.504  & 1.089  & \textbf{0.465 } & \textbf{0.953 } & 0.613  & 1.226  & \textbf{0.516 } & \textbf{1.066 } & 0.513  & 1.130  & \textbf{0.458 } & \textbf{0.946 } \\
    \multicolumn{1}{c|}{} & 336   & 0.521  & 1.112  & \textbf{0.480 } & \textbf{0.976 } & 0.624  & 1.221  & \textbf{0.555 } & \textbf{1.080 } & 0.521  & 1.129  & \textbf{0.471 } & \textbf{0.975 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Umass4\end{sideways}}} & 1     & 0.255  & 0.654  & \textbf{0.206 } & \textbf{0.504 } & 0.354  & 0.719  & \textbf{0.322 } & \textbf{0.674 } & 0.222  & 0.548  & \textbf{0.205 } & \textbf{0.498 } \\
    \multicolumn{1}{c|}{} & 6     & 0.288  & 0.622  & \textbf{0.265 } & \textbf{0.561 } & 0.430  & 0.846  & \textbf{0.386 } & \textbf{0.773 } & 0.271  & 0.660  & \textbf{0.240 } & \textbf{0.580 } \\
    \multicolumn{1}{c|}{} & 12    & 0.288  & 0.696  & \textbf{0.287 } & \textbf{0.666 } & 0.466  & 0.869  & \textbf{0.430 } & \textbf{0.806 } & 0.270  & 0.648  & \textbf{0.254 } & \textbf{0.599 } \\
    \multicolumn{1}{c|}{} & 24    & 0.283  & 0.698  & \textbf{0.270 } & \textbf{0.659 } & 0.451  & 0.860  & \textbf{0.429 } & \textbf{0.817 } & 0.289  & 0.680  & \textbf{0.263 } & \textbf{0.621 } \\
    \multicolumn{1}{c|}{} & 36    & 0.341  & 0.828  & \textbf{0.286 } & \textbf{0.661 } & 0.519  & 0.892  & \textbf{0.442 } & \textbf{0.830 } & 0.304  & 0.723  & \textbf{0.276 } & \textbf{0.656 } \\
    \multicolumn{1}{c|}{} & 48    & 0.342  & 0.832  & \textbf{0.341 } & \textbf{0.801 } & 0.477  & 0.888  & \textbf{0.439 } & \textbf{0.837 } & 0.290  & 0.698  & \textbf{0.265 } & \textbf{0.641 } \\
    \multicolumn{1}{c|}{} & 60    & 0.323  & 0.738  & \textbf{0.303 } & \textbf{0.732 } & 0.522  & 0.899  & \textbf{0.492 } & \textbf{0.843 } & 0.283  & 0.693  & \textbf{0.257 } & \textbf{0.605 } \\
    \multicolumn{1}{c|}{} & 72    & 0.311  & 0.761  & \textbf{0.300 } & \textbf{0.665 } & 0.485  & 0.886  & \textbf{0.484 } & \textbf{0.830 } & 0.299  & 0.715  & \textbf{0.269 } & \textbf{0.638 } \\
    \multicolumn{1}{c|}{} & 168   & 0.375  & 0.897  & \textbf{0.353 } & \textbf{0.790 } & 0.527  & 0.915  & \textbf{0.484 } & \textbf{0.850 } & 0.316  & 0.732  & \textbf{0.292 } & \textbf{0.653 } \\
    \multicolumn{1}{c|}{} & 336   & 0.364  & 0.797  & \textbf{0.363 } & \textbf{0.755 } & \textbf{0.475 } & 0.887  & 0.493  & \textbf{0.858 } & 0.328  & 0.740  & \textbf{0.307 } & \textbf{0.670 } \\
    \midrule
    \multicolumn{2}{c||}{Avg \% Imp} & /     & /     & \textbf{6.14\%} & \textbf{9.24\%} & /     & /     & \textbf{10.07\%} & \textbf{9.85\%} & /     & /     & \textbf{7.88\%} & \textbf{13.25\%} \\
    \bottomrule
    \end{tabular}%
  % \label{tab:addlabel}%
\end{table*}%


% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{Add caption}
%     \begin{tabular}{cc||cccccccccccc}
%     \toprule
%     \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TS-mixer} & \multicolumn{2}{c}{ +ours} \\
%     \midrule

%   \label{tab:addlabel}%
% \end{table}%


==> src/table/table_final.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
  \centering
  \caption{Comparison of forecasting errors between the baselines and our method}
        \begin{tabular}{cc||cccccccccccc}
    \toprule
    \multicolumn{2}{c}{Method} & \multicolumn{2}{c}{Crossformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{Etsformer} & \multicolumn{2}{c}{ +ours} & \multicolumn{2}{c}{TS-mixer} & \multicolumn{2}{c}{ +ours} \\
    \midrule
    \multicolumn{2}{c}{Metric} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} & \multicolumn{1}{l}{MAE} & \multicolumn{1}{l}{MAPE`} \\
    \midrule
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}Ampds2\end{sideways}}} & 1     & 0.520  & 1.074  & \textbf{0.352 } & \textbf{0.669 } & 0.446  & 0.916  & \textbf{0.434 } & \textbf{0.895 } & 0.393  & 0.769  & \textbf{0.379 } & \textbf{0.679 } \\
    \multicolumn{1}{c|}{} & 6     & 0.476  & 0.939  & \textbf{0.400 } & \textbf{0.777 } & 0.496  & 1.009  & \textbf{0.448 } & \textbf{0.884 } & 0.425  & 0.885  & \textbf{0.396 } & \textbf{0.738 } \\
    \multicolumn{1}{c|}{} & 12    & 0.491  & 1.038  & \textbf{0.402 } & \textbf{0.776 } & 0.505  & 1.032  & \textbf{0.452 } & \textbf{0.893 } & 0.434  & 0.923  & \textbf{0.402 } & \textbf{0.757 } \\
    \multicolumn{1}{c|}{} & 24    & 0.480  & 0.977  & \textbf{0.407 } & 0.775  & 0.502  & 1.032  & \textbf{0.452 } & \textbf{0.892 } & 0.435  & 0.925  & \textbf{0.404 } & \textbf{0.762 } \\
    \multicolumn{1}{c|}{} & 36    & 0.508  & 1.092  & \textbf{0.417 } & \textbf{0.810 } & 0.508  & 1.039  & \textbf{0.458 } & \textbf{0.916 } & 0.439  & 0.930  & \textbf{0.410 } & \textbf{0.780 } \\
    \multicolumn{1}{c|}{} & 48    & 0.515  & 1.136  & \textbf{0.417 } & \textbf{0.821 } & 0.509  & 1.040  & \textbf{0.459 } & \textbf{0.911 } & 0.441  & 0.930  & \textbf{0.410 } & \textbf{0.776 } \\
    \multicolumn{1}{c|}{} & 60    & 0.491  & 0.991  & \textbf{0.417 } & \textbf{0.778 } & 0.511  & 1.041  & \textbf{0.460 } & \textbf{0.908 } & 0.440  & 0.921  & \textbf{0.411 } & \textbf{0.769 } \\
    \multicolumn{1}{c|}{} & 72    & 0.513  & 1.111  & \textbf{0.421 } & \textbf{0.774 } & 0.510  & 1.037  & \textbf{0.462 } & \textbf{0.918 } & 0.445  & 0.938  & \textbf{0.417 } & \textbf{0.802 } \\
    \multicolumn{1}{c|}{} & 168   & 0.446  & 0.891  & \textbf{0.431 } & \textbf{0.837 } & 0.512  & 1.033  & \textbf{0.470 } & \textbf{0.902 } & 0.455  & 0.957  & \textbf{0.425 } & \textbf{0.798 } \\
    \multicolumn{1}{c|}{} & 336   & 0.472  & 0.954  & \textbf{0.439 } & \textbf{0.772 } & 0.525  & 1.035  & \textbf{0.512 } & \textbf{0.929 } & 0.470  & 0.969  & \textbf{0.438 } & \textbf{0.814 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}UK-Dale1\end{sideways}}} & 1     & 0.370  & 0.789  & \textbf{0.349 } & \textbf{0.705 } & 0.491  & 0.962  & \textbf{0.467 } & \textbf{0.943 } & 0.362  & \textbf{0.694 } & 0.361  & 0.697  \\
    \multicolumn{1}{c|}{} & 6     & \textbf{0.425 } & \textbf{0.828 } & 0.428  & 0.862  & 0.566  & 1.066  & \textbf{0.540 } & \textbf{1.037 } & 0.446  & 0.868  & \textbf{0.427 } & \textbf{0.817 } \\
    \multicolumn{1}{c|}{} & 12    & 0.464  & 0.937  & \textbf{0.447 } & \textbf{0.911 } & 0.591  & 1.095  & \textbf{0.553 } & \textbf{1.054 } & 0.457  & 0.888  & \textbf{0.435 } & \textbf{0.831 } \\
    \multicolumn{1}{c|}{} & 24    & 0.456  & 0.869  & \textbf{0.450 } & \textbf{0.869 } & 0.598  & 1.107  & \textbf{0.553 } & \textbf{1.081 } & 0.469  & 0.907  & \textbf{0.443 } & \textbf{0.831 } \\
    \multicolumn{1}{c|}{} & 36    & 0.477  & 0.940  & \textbf{0.451 } & \textbf{0.827 } & 0.609  & 1.134  & \textbf{0.559 } & \textbf{1.082 } & 0.485  & 0.938  & \textbf{0.454 } & \textbf{0.855 } \\
    \multicolumn{1}{c|}{} & 48    & 0.476  & 0.979  & \textbf{0.458 } & \textbf{0.907 } & 0.595  & 1.110  & \textbf{0.550 } & \textbf{1.067 } & 0.464  & 0.916  & \textbf{0.443 } & \textbf{0.850 } \\
    \multicolumn{1}{c|}{} & 60    & 0.467  & 0.915  & \textbf{0.460 } & \textbf{0.911 } & 0.593  & 1.123  & \textbf{0.561 } & \textbf{1.082 } & 0.466  & 0.923  & \textbf{0.450 } & \textbf{0.877 } \\
    \multicolumn{1}{c|}{} & 72    & 0.482  & 0.977  & \textbf{0.466 } & \textbf{0.946 } & 0.593  & 1.129  & \textbf{0.548 } & \textbf{1.064 } & 0.470  & 0.931  & \textbf{0.449 } & \textbf{0.872 } \\
    \multicolumn{1}{c|}{} & 168   & 0.493  & 1.078  & \textbf{0.464 } & \textbf{0.975 } & 0.585  & 1.135  & \textbf{0.529 } & \textbf{1.077 } & 0.470  & 0.949  & \textbf{0.446 } & \textbf{0.870 } \\
    \multicolumn{1}{c|}{} & 336   & 0.483  & 1.024  & \textbf{0.457 } & \textbf{0.918 } & 0.572  & 1.145  & \textbf{0.524 } & \textbf{1.075 } & 0.470  & 0.957  & \textbf{0.448 } & \textbf{0.881 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}UmassC\end{sideways}}} & 1     & 0.401  & 0.903  & \textbf{0.384 } & \textbf{0.855 } & 0.497  & 1.044  & \textbf{0.472 } & \textbf{1.023 } & 0.423  & 0.894  & \textbf{0.395 } & \textbf{0.795 } \\
    \multicolumn{1}{c|}{} & 6     & 0.466  & 0.956  & \textbf{0.426 } & \textbf{0.858 } & 0.575  & 1.171  & \textbf{0.511 } & \textbf{1.054 } & 0.484  & 1.047  & \textbf{0.439 } & \textbf{0.922 } \\
    \multicolumn{1}{c|}{} & 12    & 0.482  & 1.001  & \textbf{0.438 } & \textbf{0.900 } & 0.601  & 1.204  & \textbf{0.520 } & \textbf{1.083 } & 0.493  & 1.064  & \textbf{0.441 } & \textbf{0.908 } \\
    \multicolumn{1}{c|}{} & 24    & 0.499  & 1.053  & \textbf{0.468 } & \textbf{0.999 } & 0.597  & 1.205  & \textbf{0.537 } & \textbf{1.093 } & 0.503  & 1.083  & \textbf{0.451 } & \textbf{0.947 } \\
    \multicolumn{1}{c|}{} & 36    & 0.499  & 1.073  & \textbf{0.451 } & \textbf{0.912 } & 0.604  & 1.205  & \textbf{0.518 } & \textbf{1.075 } & 0.505  & 1.093  & \textbf{0.445 } & \textbf{0.901 } \\
    \multicolumn{1}{c|}{} & 48    & 0.493  & 1.047  & \textbf{0.447 } & \textbf{0.899 } & 0.610  & 1.221  & \textbf{0.524 } & \textbf{1.082 } & 0.502  & 1.094  & \textbf{0.452 } & \textbf{0.945 } \\
    \multicolumn{1}{c|}{} & 60    & 0.497  & 1.026  & \textbf{0.457 } & \textbf{0.951 } & 0.609  & 1.220  & \textbf{0.547 } & \textbf{1.113 } & 0.509  & 1.110  & \textbf{0.457 } & \textbf{0.971 } \\
    \multicolumn{1}{c|}{} & 72    & 0.508  & 1.106  & \textbf{0.468 } & \textbf{0.977 } & 0.622  & 1.235  & \textbf{0.530 } & \textbf{1.088 } & 0.509  & 1.109  & \textbf{0.457 } & \textbf{0.955 } \\
    \multicolumn{1}{c|}{} & 168   & 0.501  & 1.068  & \textbf{0.462 } & \textbf{0.940 } & 0.619  & 1.231  & \textbf{0.530 } & \textbf{1.093 } & 0.514  & 1.125  & \textbf{0.456 } & \textbf{0.942 } \\
    \multicolumn{1}{c|}{} & 336   & 0.519  & 1.079  & \textbf{0.487 } & \textbf{1.021 } & 0.627  & 1.234  & \textbf{0.545 } & \textbf{1.083 } & 0.519  & 1.130  & \textbf{0.474 } & \textbf{0.998 } \\
    \midrule
    \multicolumn{1}{c|}{\multirow{10}[2]{*}{\begin{sideways}UmassD\end{sideways}}} & 1     & \textbf{0.263 } & 0.645  & 0.291  & \textbf{0.601 } & \textbf{0.339 } & 0.717  & 0.357  & \textbf{0.707 } & 0.221  & 0.547  & \textbf{0.198 } & \textbf{0.478 } \\
    \multicolumn{1}{c|}{} & 6     & 0.279  & \textbf{0.637 } & \textbf{0.275 } & 0.647  & 0.420  & 0.824  & \textbf{0.411 } & \textbf{0.796 } & 0.265  & 0.646  & \textbf{0.240 } & \textbf{0.574 } \\
    \multicolumn{1}{c|}{} & 12    & 0.311  & 0.745  & \textbf{0.281 } & \textbf{0.668 } & 0.473  & 0.877  & \textbf{0.425 } & \textbf{0.813 } & 0.270  & 0.650  & \textbf{0.255 } & \textbf{0.609 } \\
    \multicolumn{1}{c|}{} & 24    & 0.306  & 0.687  & \textbf{0.280 } & \textbf{0.669 } & 0.469  & 0.869  & \textbf{0.424 } & \textbf{0.814 } & 0.283  & 0.673  & \textbf{0.260 } & \textbf{0.611 } \\
    \multicolumn{1}{c|}{} & 36    & 0.323  & 0.786  & \textbf{0.287 } & \textbf{0.652 } & 0.499  & 0.883  & \textbf{0.459 } & \textbf{0.821 } & 0.292  & 0.707  & \textbf{0.263 } & \textbf{0.625 } \\
    \multicolumn{1}{c|}{} & 48    & 0.328  & 0.774  & \textbf{0.309 } & \textbf{0.677 } & 0.492  & 0.891  & \textbf{0.456 } & \textbf{0.827 } & 0.285  & 0.691  & \textbf{0.261 } & \textbf{0.624 } \\
    \multicolumn{1}{c|}{} & 60    & 0.308  & 0.731  & \textbf{0.302 } & \textbf{0.705 } & 0.491  & 0.885  & \textbf{0.473 } & \textbf{0.845 } & 0.293  & 0.712  & \textbf{0.262 } & \textbf{0.629 } \\
    \multicolumn{1}{c|}{} & 72    & 0.330  & 0.782  & \textbf{0.298 } & \textbf{0.693 } & 0.488  & 0.880  & \textbf{0.470 } & \textbf{0.842 } & 0.297  & 0.711  & \textbf{0.271 } & \textbf{0.640 } \\
    \multicolumn{1}{c|}{} & 168   & 0.364  & 0.867  & \textbf{0.349 } & \textbf{0.731 } & 0.514  & 0.912  & \textbf{0.471 } & \textbf{0.862 } & 0.314  & 0.730  & \textbf{0.291 } & \textbf{0.659 } \\
    \multicolumn{1}{c|}{} & 336   & \textbf{0.360 } & 0.838  & 0.368  & \textbf{0.773 } & 0.502  & 0.906  & \textbf{0.479 } & \textbf{0.861 } & 0.322  & 0.735  & \textbf{0.308 } & \textbf{0.677 } \\
    \midrule
    \multicolumn{2}{c||}{Avg \% Imp} & /     & /     & \textbf{7.85\%} & \textbf{11.67\%} & /     & /     & \textbf{8.14\%} & \textbf{7.56\%} & /     & /     & \textbf{7.27\%} & \textbf{11.49\%} \\
    \bottomrule
    \end{tabular}%
    \label{table:main result}
\end{table*}%


==> src/table/without_msp_acc.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \setlength{\tabcolsep}{1.8pt}
  \caption{Ablation without Response Loss: the average metric which horizon in \qh{$[1,6,12,24,36,48,60,72,168,336]$.}}
    \begin{tabular}{c||cccccccc}
    \toprule
    \multicolumn{1}{c}{Method} & \multicolumn{2}{c}{Origin} & \multicolumn{3}{c}{w/o MSP} & \multicolumn{3}{c}{+ours} \\
    \midrule
    \multicolumn{1}{c}{Metric} & MAE   & MAPE$^\prime$ & MAE   & MAPE$^\prime$ & \cxrev{ACC}   & MAE   & MAPE$^\prime$ & \cxrev{ACC} \\
    \midrule
    \midrule
    Ampds2 & 0.491  & 1.005  & 0.495  & 0.999  & \cxrev{80.3\%} & \textbf{0.452 } & \textbf{0.883 } & \cxrev{\textbf{85.3\%}} \\
    UK-Daleh1 & 0.576  & 1.101  & 0.574  & 1.089  & \cxrev{88.4\%} & \textbf{0.535 } & \textbf{1.050 } & \cxrev{\textbf{91.0\%}} \\
    UmassC & 0.594  & 1.193  & 0.584  & 1.177  & \cxrev{86.1\%} & \textbf{0.518 } & \textbf{1.060 } & \cxrev{\textbf{88.8\%}} \\
    UmassD & 0.471  & 0.866  & 0.453  & 0.850  & \cxrev{94.1\%} & \textbf{0.436 } & \textbf{0.810 } & \cxrev{\textbf{96.0\%}} \\
    \bottomrule
    \end{tabular}%
  \label{tab:blation without MSP}%
\end{table}%

